DocLens: Multi-aspect Fine-grained Evaluation for Medical Text Generation

Medical text generation aims to assist with administrative work and highlight salient information to support decision-making. To reflect the specific requirements of medical text, in this paper, we propose a set of metrics to evaluate the completeness, conciseness, and attribution of the generated text at a fine-grained level. The metrics can be computed by various types of evaluators including instruction-following (both proprietary and open-source) and supervised entailment models. We demonstrate the effectiveness of the resulting framework, DocLens, with three evaluators on three tasks: clinical note generation, radiology report summarization, and patient question summarization. A comprehensive human study shows that DocLens exhibits substantially higher agreement with the judgments of medical experts than existing metrics. The results also highlight the need to improve open-source evaluators and suggest potential directions.

==> 3_eval_framework_orig.tex <==

\section{Evaluation Framework of \modelname}
\label{sec:eval_framework}

To design an evaluation pipeline tailored for medical text generation, we identify the important evaluation aspects (\S\ref{sec:aspects}), design a set of metrics corresponding to the aspects (\S\ref{sec:metrics}), and adopt LLM as the evaluator to compute each metric with two prompt engineering techniques (\S\ref{sec:framework}).


\subsection{Evaluation Aspects}
\label{sec:aspects}


In the medical domain, where decisions can have significant implications for patient health and outcomes, the accuracy and completeness of the generated text are paramount.
Compared to evaluation in general domains, there are two special characteristics of the medical domain:
(a) Every piece of information is essential. Any inaccurate or omitted information can lead to incorrect diagnoses or inappropriate treatments.
(b) The generated text is typically used in a \emph{supporting} role rather than in direct production. In healthcare, where decisions can be life-critical, the highest degree of accuracy is required. Hence, the generated text will typically be manually verified by medical experts.






\start{Aspect 1: Completeness at fine-grained level} 
We first evaluate completeness: the amount of clinically significant detail retained from the input text. This can be viewed as the recall of the generated output.
Based on characteristic (a), unlike previous work~\cite{clinical-text-summ} that scores the completeness of the whole piece of output, we are also interested in which exact important information is retained and which is omitted.
For example, as shown in \autoref{fig:eval_aspects}, 
the generated clinical note omits the past medical history of the patient and the exam result of edema in both arms.

\start{Aspect 2: Conciseness at fine-grained level} 
Following (b), to reduce the workload of medical experts, we evaluate conciseness: the amount of generated information that is both factually accurate and salient.
With concise text generated by models, medical experts can quickly capture crucial information, without spending significant time on superfluous details.
Similar to completeness evaluation, we evaluate at a fine-grained level and check which piece of generated information is crucial and which is unimportant.

\start{Aspect 3: Verifiability} 
Based on characteristic (b), to help the professionals quickly verify the generated statements, we also evaluate verifiability: the amount of generated information that is both accurate and easy to verify.
As shown in \autoref{fig:eval_aspects}, the model generates citations to the input that supports the statement about the musculoskeletal exam, which helps medical experts quickly locate the relevant context and verify the generated information.



\start{Discussion of other aspects} 
There are other evaluation aspects for text generation in general domains, such as \textbf{coherence} and \textbf{fluency}~\cite{zhong-etal-2022-towards,ALCE}, where coherence evaluates whether all the sentences form a coherent body and fluency evaluates whether each generated sentence is fluent and natural.
These aspects are less emphasized in the medical domain since they do not directly impact treatment outcomes.

To ensure the generated text is accurate, many existing methods evaluate \textbf{factual consistency}\cite{fever,multifc,clinical-text-summ}, which compares the factual statements in the generated text and the input.
Among our proposed aspects, conciseness and interpretability both incorporate the need for factual consistency.
In addition to the factuality of generated statements, conciseness further evaluates whether the statements are important and interpretability judges whether they are also easy to verify.



\begin{figure}[!t]
\centering
    \centering
    \includegraphics[width=0.9\linewidth]{figures/entail_diagram.pdf}
    \upv
    \vspace{-0.1cm}
    \caption{To conduct a multi-aspect evaluation, we verify the existence of entailment relations among the input (e.g., patient-doctor dialogue), output (e.g., generated clinical note), and reference (e.g., reference note).
    }
    \label{fig:entail_diagram}
    \downv
    \vspace{-0.25cm}
\end{figure}

\vspace{-0.1cm}
\begin{figure*}[t]
\centering
    \centering
    \includegraphics[width=0.95\linewidth]{figures/metrics_examples.pdf}
    \upv
    \caption{Illustration of the metrics of \modelname for medical evaluation:
    \textcolor{textRed}{\textbf{Claim Recall}} measures the proportion of claims from the reference that can be entailed by the generated output. 
    \textcolor{textYellow}{\textbf{Claim Precision}} measures the proportion of claims from the output that can be entailed by the reference. 
    \textcolor{textBlue}{\textbf{Citation Recall}} measures the proportion of output sentences that can be entailed by their corresponding citations. 
    \textcolor{textBlue}{\textbf{Citation Precision}} measures the proportion of citations that factually support the associated sentence.}
    \label{fig:eval_pipeline}
    \downv
    \vspace{-0.2cm}
\end{figure*}



\subsection{Evaluation Metrics}
\label{sec:metrics}


To conduct evaluation, as shown in \autoref{fig:entail_diagram}, we formulate the evaluation of the proposed aspects as the verification of the entailment relations among the input, output, and reference.
For instance, we judge the degree of completeness by the amount of information in the reference that can be entailed from the output. 
With this formulation, we design the following metrics that can be computed by an evaluator model, which can either be a supervised NLI model or a large language model.
The illustration of each metric is shown in \autoref{fig:eval_pipeline}.

\start{Completeness evaluation: claim recall} 
We use claim recall to evaluate the completeness of the output, which corresponds to the relation ``Output$\Rightarrow$Reference'' in \autoref{fig:entail_diagram}.
As shown in \autoref{fig:eval_pipeline}, we first break down the reference into a list of claims using GPT-4~\cite{openai2023gpt4}, where each claim states a fact in the reference.
Then we apply the evaluator to judge whether each claim is entailed by the generated output. Claim recall is computed by the percentage of claims that can be entailed by the output.

The concept of claim recall parallels the definition provided in ALCE \cite{ALCE}, with the following difference:
ALCE only requires the output to follow the key reasoning steps in the reference and hence restricts the extraction to three claims per instance.
In contrast, since a clinical note should cover all important details, we prompt the model to generate claims that encapsulate all factual information in the reference.

\start{Conciseness evaluation: claim precision} 
To evaluate conciseness, assuming that the reference only contains important information, we define claim precision, which aligns with the "Reference$\Rightarrow$Output" relation in \autoref{fig:entail_diagram}.
Similar to claim recall, we generate a list of claims based on the output and then apply the evaluator to determine whether the reference entails each claim. Claim precision is defined as the proportion of claims that can be entailed by the reference. 

\start{Verifiability evaluation: citation recall} 
There exist multiple methods to evaluate verifiability. Here we train or prompt the model to generate citations from the input for each generated statement and evaluate the citation quality.
Following existing work \cite{liu2023evaluating,ALCE}, we first evaluate whether the combination of cited sentences can fully entail each generated statement.
The corresponding metric is citation recall: the percentage of generated statements that can be entailed by the concatenation of their citations.


\start{Verifiability evaluation: citation precision} 
We also calculate the precision for each citation (0 or 1) and average over all the citations in the output.
If a sentence can be supported by its citations, the citations pertinent to this sentence will have citation precision = 1, and other irrelevant citations will have citation precision = 0.
For instance, in \autoref{fig:eval_pipeline}, the output sentence cites conversational turns ``\texttt{[21][22][23]}'' in the input, but only \texttt{[21]} and \texttt{[22]} are pertinent to the output. So \texttt{[21]} and \texttt{[22]} will have citation precision = 1 and \texttt{[23]} will have citation precision = 0.
If a sentence cannot be entailed by its citations, we set citation precision = 0 for all its citations.













\subsection{Power \modelname with LLMs}
\label{sec:framework}

Large language models (LLMs) have shown remarkable generalization and instruction-following abilities in various domains, including the medical domain. In this section, we design a framework that powers \modelname with LLMs.

To compute claim recall and claim precision, we prompt the LLM evaluator to generate ``1'' or ``0'' for each claim based on whether they can be entailed by the reference or output.
As for citation recall and precision, we prompt the evaluator to generate both the entailment prediction and the relevant citation indexes in a single call. 
In the example of \autoref{fig:eval_pipeline}, where the citations ``\texttt{[21][22][23]}'' support the generated statement but \texttt{[23]} is irrelevant, the LLM evaluator should output ``1'' for the entailment prediction and ``\texttt{[21][22]}'' as the relevant citations.

We further investigate different prompt styles to improve the LLM evaluator's entailment ability and thereby improve the evaluation quality, where the final prompt template is provided in \autoref{tab:nli_prompt}:

(1) \textbf{Generation with Structure}.
Existing research has observed that large language models tend to generate more accurate output when they are prompted to generate in a structured format, such as logic representations, or pseudo code \cite{mishra2023pseudocode}.
With the same high-level idea, we prompt the LLM evaluator to generate the entailment prediction in a JSON dictionary.

(2) \textbf{Chain-of-Thought}.
Chain-of-thought (CoT) prompts the model to generate a series of intermediate reasoning steps, which has shown to be effective for LLMs~\cite{cot}.
Following this idea, we prompt the LLM evaluator to generate the explanation before the entailment prediction. 

We conduct experiments to demonstrate the effectiveness of LLM evaluators.
Results in \autoref{tab:NLI} and \autoref{tab:NLI_3way} show that with the combination of generation in JSON and CoT, GPT-4 outperforms existing NLI models on NLI datasets.
\autoref{tab:human_spearman} further demonstrates that compared to existing NLI models, the GPT-4 evaluator achieves higher agreement with human on the computation of claim recall.


==> arxiv_3_fact_eval.tex <==
\input{tables/formulation}



\section{Evaluation Aspects of Medical Generation}
\label{sec:entailment}

In the medical domain, it is less of our interest to generate text that is fluent or \emph{appears} informative. The most important requirements are that the generated text contains well-supported statements (and ideally accurate citations). In other words, the generated text must be factually supported by the input. Any inaccurate or omitted information can lead to incorrect diagnoses and inappropriate treatments. Hence we evaluate whether statements of the generated text are supported and whether the provided facts are missing in the generated text. 

\subsection{Formulation of Factuality Relations}
\autoref{fig:entail_diagram} illustrates factuality relationships among the input, output, and reference. Evaluation of them can be formulated as entailment problems: 

\noindent\textbf{Output$\Rightarrow$Reference} The system output should be able to support statements in the reference. In other words, if a statement is present in the reference, it should be entailed from the output. This is important because it ensures that the output is factually consistent with the reference and can be used to verify the \emph{recall} of the system. %

\noindent\textbf{Reference$\Rightarrow$Output} In reverse, statements in the output should be entailed from the reference, i.e., the output does not contain irrelevant information. This also ensures factual consistency and can be used to verify the \emph{precision} of the system.

\noindent\textbf{Input$\Rightarrow$Output} In the real-word scenario, the reference is oftentimes unavailable. Therefore, it is important for the system output to have \emph{verifiability}~\cite{liu2023evaluating}, that is, (1) statements in the output should have granular citations to the input; (2) each citation should be able to entail the associated statement.

\input{tables/NLI}

\begin{figure}[!t]
\centering
    \centering
    \includegraphics[width=0.9\linewidth]{figures/entail_diagram.pdf}
    \upv
    \caption{Factuality relations among input (e.g., patient-doctor dialogues), output (e.g., reference notes), and reference are formulated as entailment problems.}
    \label{fig:entail_diagram}
    \downv
\end{figure}




\subsection{Entailment with GPT-4}
With the formulation of factuality evaluation as entailment, we explore using GPT-4 for entailment evaluation and compare it with the state-of-the-art entailment models.
 We design a set of prompts that elicit entailment judgments from GPT-4, as illustrated by the example in \autoref{tab:nli_prompt}.



(1) \textbf{Generation with Structure}.
Existing research has observed that large language models generate more accurate output when they are prompted to generate in a structured format, such as JSON files, logic representations, or structured text~\cite{white2023prompt}.
Following their observation, we prompt the GPT-4 evaluator to generate the entailment prediction in a JSON dictionary.
The prompt style is denoted as ``Json''.

(2) \textbf{Chain-of-Thought}.
Chain-of-thought reasoning (CoT) generates a series of intermediate reasoning steps and has shown to be effective for LLMs~\cite{cot}.
We prompt GPT-4 to generate the explanation before the entailment prediction. 
The prompt style is denoted as ``CoT''.



\start{Experiments} We conduct experiments on two prevalent natural language inference (NLI) datasets: ANLI~\cite{ANLI} and MedNLI~\cite{MedNLI}.
To evaluate binary factual consistency, we merge two NLI labels ``\emph{neutral}'' and ``\emph{contradiction}'' into one class, denoting inconsistency between a premise-hypothesis pair.


Table~\ref{tab:NLI} compares GPT-4 with TRUE~\cite{TRUE}, which is a T5-11B~\cite{raffel2023exploring} model fine-tuned on a collection of NLI datasets. TRUE targets factual correctness and has been used by previous works in similar
context~\cite{bohnet2023attributed,gao-etal-2023-rarr,ALCE}. GPT-4 significantly outperforms TRUE on both datasets. Comparing different prompt styles, we observe that JSON output format and few-shot examples clearly improve GPT-4 entailment accuracy. CoT also helps the model achieve the best average accuracy.


We further compare GPT-4 with supervised state-of-the-art models on MedNLI in Table~\ref{tab:NLI_3way}. 
By combining in-context learning (few-shot and CoT) and JSON output format, GPT-4 substantially outperforms all supervised models. 
Therefore, we choose to use GPT-4 for entailment evaluation.


\input{tables/MedNLI_3way}

\begin{figure*}[t]
\centering
    \centering
    \includegraphics[width=0.9\linewidth]{figures/metrics_examples.pdf}
    \upv
    \caption{Illustration of proposed evaluation metrics for medical text generations:
    (1) \textbf{Claim Recall} measures the proportion of claims from the reference that can be entailed by the generated output. 
    (2) \textbf{Claim Precision} measures the proportion of claims from the output that can be entailed by the reference. 
    (3) \textbf{Citation Recall} measures the proportion of output sentences that can be entailed by their corresponding citations. 
    (4) \textbf{Citation Precision} measures the proportion of citations that factually support the associated sentence.}
    \label{fig:eval_pipeline}
    \downv
\end{figure*}




==> arxiv_4_eval_pipeline.tex <==


\section{Evaluation Metrics based on GPT-4}
\label{sec:gpt-4-metrics}

Section \ref{sec:entailment} describes our formulation of evaluating factual consistency as entailment and demonstrates the effectiveness of GPT-4 for entailment.
Here, we introduce a set of metrics that leverage GPT-4 to evaluate factuality relations shown in \autoref{fig:eval_pipeline}.%

\noindent\textbf{Claim recall}: We first break down the reference into a list of claims using GPT-4. Each claim states a fact in the reference.
Then we ask GPT-4 to judge whether each claim is entailed by the generated output. Claim recall is computed by the percentage of claims that can be entailed by the output.
It corresponds to the relation ``Output$\Rightarrow$Reference'' described in Section \ref{sec:entailment}.

The concept of claim recall parallels the definition provided in ALCE \cite{ALCE}, with notable differences in our approach: ALCE restricts the extraction to three claims per instance, we encourage the model to generate claims encapsulating all factual information in the reference.
Additionally, while ALCE uses a supervised model for the entailment judgement, we use GPT-4.

\noindent\textbf{Claim precision}: Similar to claim recall, our initial step involves generating a list of claims based on the output, followed by the utilization of GPT-4 to determine whether the reference entails each claim. Claim precision is quantified as the proportion of claims that can be entailed by the reference, aligning with the "Reference$\Rightarrow$Output" relation in Section \ref{sec:entailment}. In contrast to claim recall, claim precision exposes statements unsupported by the reference, thereby serving as a metric for hallucination detection. To our best understanding, we are the first to evaluate claim precision in text generation.

\noindent\textbf{Citation recall}: Following ALCE \cite{ALCE}, we prompt LLMs to generate citations from the input for each generated sentence.
To assess the citation quality, for each sentence in the output, we concatenate the cited sentences and ask GPT-4 to judge whether the cited sentences can fully entail the generated sentence.
Citation recall is thus defined as the percentage of sentences that can be entailed by their citations.

\noindent\textbf{Citation precision}: 
We also calculate the citation precision for each citation (0 or 1) and average over all citations in the output.
If a sentence can be supported by its citations, the citations pertinent to this sentence will have citation precision = 1, and other irrelevant citations will have citation precision = 0.
For instance, in \autoref{fig:eval_pipeline}, the output sentence cites [21][22][23], but only [21] and [22] are pertinent to the output. So [21] and [22] will have citation precision = 1 and [23] will have citation precision = 0.
If a sentence cannot be entailed by its citations, we set citation precision = 0 for all its citations.

In contrast to ALCE, which leaves one citation out at a time and verifies if the entailment relation still satisfies, we prompt GPT-4 in a single call to generate all citation numbers that support the output sentence. We have observed that this method performs on par with the leave-one-out strategy while significantly accelerating the evaluation speed. 
The exact prompt is provided in the Appendix.
Citation recall and precision correspond to the "Input$\Rightarrow$Output" relation in Section \ref{sec:entailment}.



==> note_exp.tex <==
\section{Clinical Note Generation Experiments}

\subsection{Models}

\start{Supervised Models}
Use the outputs in the repo of ACI-BENCH. Introduce the section and full settings here.

\start{Large Language Models}
GPT-3.5 and GPT-4. 
Explain the few-shot examples.
Two settings for note generation: per-section generation and full-note generation.

\subsection{Note Generation Results}
\autoref{tab:ACI_combine}.

Introduce the best model under each of our metrics and explain why (e.g., section models always generate longer outputs so they have high recall score and low claim prec scores for object sections)

If there's mismatch between existing metrics and GPT-4 eval, explain why -- could be cases where we can show GPT-4 eval is better than existing metrics.


\input{tables/ACI_combine}


==> orig_3_setting.tex <==
\section{Evaluation Settings}

\subsection{Evaluation Metrics}
First, explain that factuality and self-consistency (citation quality) are the most important aspects.

Then formulate both metrics as entailment problems.



\start{Correctness} Claim Recall. The evaluation of citation recall can be viewed as a 2-way classification task, where the label classes are ``entailment'' and ``neutral''.

\start{Citation quality} Citation recall and precision. Similarly, both citation recall and precision can be viewed as 2-way classification, with ``entailment'' and ``neutral'' as label classes.

\subsection{Evaluation Pipeline}
Figure~\ref{fig:eval_pipeline}.

We first follow ALCE and use TRUE~\cite{TRUE} to evaluate correctness and citation quality. Then we further investigate using LLM to compute these metrics.
We will introduce the prompt for both entailment problems.


==> orig_4.5_datasets.tex <==
\section{Experimental Setup}

\subsection{Evaluation Tasks}
We focus on two representing tasks: note generation and report summarization.

\start{Note Generation}
In note generation, the input is a dialogue between a doctor and a patient, and the goal is to generate a clinical note base on the dialogue \cite{aci-bench,mts-dialog}. Each sentence in the clinical note should cite at least one conversational turn in the input dialogue that supports the sentence.

We will introduce the prompts for note generation models after the details are fixed.

\start{Report Summarization}
In report summarization, the input is the background or findings section of a medical report, and the goal is to generate a summary (called an Impression section) that contains the key observations and conclusions \cite{radadapt}.
Similarly, each sentence should cite at least one sentence in the input report.

We will introduce the prompts for report summarization models after the details are fixed.

\subsection{Datasets}
We conduct experiments on the ACI-BENCH~\cite{aci-bench} datasets for the evaluation of note generation and use MIMIC-III~\cite{radadapt} for report summarization.


==> orig_4_improve_llm.tex <==
\section{Improving LLM Evaluators}
We investigate several potential methods to improve LLMs' entailment ability and thereby improve the evaluation quality.

\subsection{Generation with Structure}
For the evaluation of correctness and citation quality, we prompt the LLM evaluators to generate the entailment prediction in a JSON dictionary.
The prompt style is denoted as ``Json''.

\subsection{Chain-of-Thought}
We prompt the LLM evaluators to generate the explanation before the entailment prediction. 
The prompt style is denoted as ``Json+CoT''.

\subsection{Others (TBD)}
We will try other methods to improve the entailment ability, such as \textbf{InlineSearch}, where we allow LLMs to call “search” during the generation process. In principle, this function helps the evaluator focus on the most relevant information in the input.


==> orig_5_entailment.tex <==


\subsection{Evaluation Qualities Analysis}
\start{Setup} To select the examples to evaluate, we first use several different LLM evaluators to evaluate GPT-4-32k (per-section generation, 2-shot) on ACI-BENCH and MIMIC-III using several different evaluators. 
We use the same set of subclaims for the evaluation of claim recall.
Then we randomly sample 120 sentences where at least two evaluators make different entailment predictions.
Among these 120 sentences, we share 20 among 5 human evaluators, and evenly assign the other 100 to each of the 5 evaluators. Namely, each human evaluator is assigned 40 examples in total.

To compute the accuracy of each evaluator, we consider human evaluations as the ground truth and compute the accuracy of each model. For the shared 20 examples, we use the majority vote to obtain ground truth labels.

We also inspect the agreement among human evaluators by computing Fleiss’ Kappa over 5 evaluators on the 20 shared sentences.

\start{Evaluation of Claim Recall}
The accuracy of claim recall evaluation on note generation is shown in Table~\ref{tab:claim_acc}. We will also work on the report summarization evaluation quality analysis under the same setting.

\start{Agreement among different evaluators}
In addition to the accuracy, we also compute the Fleiss' Kappa score so that we can directly compare the agreement between each LLM evaluator and human and the agreement among humans.
The results are in Table~\ref{tab:claim_agreement}.


==> orig_5_eval_tasks.tex <==


\section{Medical Text Generation Tasks}
\label{sec:tasks}
We apply the proposed evaluation metrics in two representative medical text generation tasks: clinical note generation~\cite{aci-bench} and medical report summarization~\cite{radadapt}. 

\subsection{Clinical Note Generation}
\start{Task Definition and Dataset}
Clinical note generation is defined as generating a ``SOAP'' note given a dialogue between a doctor and a patient~\cite{aci-bench,mts-dialog}. 
A SOAP note consists of the Subjective, Objective Exam, Objective Results, and Assessment and Plan sections.\footnote{\href{https://www.ncbi.nlm.nih.gov/books/NBK482263/}{ncbi.nlm.nih.gov/books/NBK482263/}} 
We conduct experiments on the ACI-BENCH dataset~\cite{aci-bench}. The details can be found in \autoref{sec:exp_details} and a test sample is shown in \autoref{tab:aci_example}.


\start{Metrics}
Beside the metrics we proposed (Section \ref{sec:metrics}), we compare the following metrics that are commonly used in the existing research~\cite{aci-bench,mts-dialog}:
\textbf{ROUGE}~\cite{rouge} computes the overlap of n-grams.
\textbf{BERTScore}~\cite{bertscore} compares the embeddings of matched tokens in the output and reference.
\textbf{BLEURT}~\cite{bleurt} trains a model to compute output-reference similarity.
\textbf{MEDCON}~\cite{aci-bench} computes the F1-score of the UMLS concepts in the output and the reference.






\subsection{Medical Report Summarization}
\start{Task Definition and Dataset}
For medical report summarization, we consider radiology report summarization on the public test set of MIMIC-III~\cite{mimic}. We follow the task definition from~\newcite{radadapt}: the input is the findings section of a radiology report, and the goal is to generate the impression section, which contains key observations and conclusions.
An example of input and reference output is shown in \autoref{tab:mimic_example}.

\start{Metrics}
In addition to the proposed metrics (\autoref{sec:metrics}), the following metrics are frequently used in existing works \cite{radadapt,medpalmm}: ROUGE, BERTScore, BLEU, and F1-RadGraph \cite{radgraph,radgraphF1}, where BLEU evaluates the overlap of 1- to 4-grams, and F1-RadGraph computes the F1 score of a predefined set of entities and relations present in radiology reports.



==> orig_6_preference.tex <==
\section{Model Preference Agreement}
One reason for conducting the evaluation is to select better generation models.
After judging the entailment ability of each evaluator, we aim to answer the next research question: Is the GPT-4 evaluator also more useful to rank generation models?

To answer this question, we compute the rankings of different pieces of generated text with both our evaluation pipeline and human preference.

\start{Setup} We evaluate a set of models on note generation and report summarization with a set of evaluators. Similar to Sec.~\ref{sec:claim_agreement}, we randomly sample $K$ test examples where at least two evaluators rank two models differently. Then we ask human evaluators to choose their preferred generated text without telling them which model generates each piece of text.
Again, we compute the agreement between each evaluator and human and among human annotators.

\start{Agreement analysis on model preference}
We are still preparing for human annotation.

Table~\ref{tab:ACI_orig} and Table~\ref{tab:ACI_TRUE} show that for the claim recall evaluation under the \textit{Subjective} section of note generation, GPT-4 ranks GPT-4-32k (section, 2-shot) higher than GPT-4 (section, 1-shot), while TRUE ranks them differently. 


==> orig_7_results.tex <==


\section{Evaluation Results}
After judging the quality of different evaluators, we are able to answer the last research question: How does every model perform on note generation and report summarization?

\start{Note generation results}

\start{Report summarization results}


==> outline.tex <==
\section{Evaluating Factual Consistency}


\section{Representative Tasks}

\subsection{Clinical Note Generation}
\paragraph{Task Definition}

\paragraph{Existing Evaluation Metrics}

\paragraph{Evaluation based on Factuality}

\subsection{Medical Report Summarization}
\paragraph{Task Definition}
\paragraph{Existing Evaluation Metrics}
\paragraph{Evaluation based on Factuality}


\section{Experiments}

\subsection{Clinical Note Generation}
\paragraph{Models}

\paragraph{Note Quality}

\paragraph{Citation Quality}


\subsection{Medical Report Summarization}
\paragraph{Summarization Quality}

\paragraph{Citation Quality}



==> summ_exp.tex <==
\section{Medical Report Summarization Experiments}
\subsection{Models}

\subsection{Medical Report Summarization Results}
Table~\ref{tab:MIMIC_orig} and Table~\ref{tab:MIMIC_full}.

\input{tables/MIMIC}


==> tables/formulation.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcc}
\toprule
\bf Evaluation Aspect & \bf Formulation & \bf Metric \\
\midrule
\midrule
Completeness & Output $\Rightarrow$ Reference & Claim Recall \\
\midrule
Conciseness & Reference $\Rightarrow$ Output & Claim precision \\
\midrule
Citation Quality & Cited input $\Rightarrow$ Output & Citation Recall \& Precision \\
\bottomrule
\end{tabular}
\caption{The entailment formulation and metrics of different aspects of factuality evaluation.}
\label{tab:formulation}
\end{table*}

